VALO: A Versatile Anytime Framework for LiDAR-based Object Detection Deep Neural Networks

This work addresses the challenge of adapting dynamic deadline requirements for LiDAR object detection deep neural networks (DNNs). The computing latency of object detection is critically important to ensure safe and efficient navigation. However, state-of-the-art LiDAR object detection DNNs often exhibit significant latency, hindering their real-time performance on resource-constrained edge platforms. Therefore, a tradeoff between detection accuracy and latency should be dynamically managed at runtime to achieve optimum results. In this paper, we introduce VALO (Versatile Anytime algorithm for LiDAR Object detection), a novel data-centric approach that enables anytime computing of 3D LiDAR object detection DNNs. VALO employs a deadline-aware scheduler to selectively process input regions, making execution time and accuracy tradeoffs without architectural modifications. Additionally, it leverages efficient forecasting of past detection results to mitigate possible loss of accuracy due to partial processing of input. Finally, it utilizes a novel input reduction technique within its detection heads to significantly accelerate execution without sacrificing accuracy. We implement VALO on state-of-the-art 3D LiDAR object detection networks, namely CenterPoint and VoxelNext, and demonstrate its dynamic adaptability to a wide range of time constraints while achieving higher accuracy than the prior state-of-the-art. Code is available athttps://github.com/CSL-KU/VALO}{github.com/CSL-KU/VALO.

==> response_letter.tex <==
\section*{Response Letter}
\subsection{Cover Letter}

Dear Reviewers, 

We would like to thank the reviewers for their helpful feedback. In response to the received feedback, we have prepared a new revision. Our changes to the paper include:
\begin{itemize}
\item Added an anytime algorithm example
 (Section~\ref{sec:background}).
\item Revised region scheduling (Section~\ref{sec:region-sched}).
\item Clarified time prediction of 3D Backbone (Section~\ref{sec:time-pred}).
\item Revised forecasting (Section~\ref{sec:forecasting}). 
\item Defined the variable \textit{c} in the Equation~\ref{eq:pose} (Section~\ref{sec:region-sched}).
\item Revised detection head optimization (Section~\ref{sec:detheadopt}). 
\item Defined the normalized accuracy metric (Section~\ref{sec:evaluation}).
%\item Mentioned that VALO applied VoxelNext does not require training (Section~\ref{sec:detheadopt}).
%\item Added deadline miss ratio figures for experiments illustrated in Figures~\ref{fig:acc2},~\ref{fig:acc3} and~\ref{fig:acc4} (Section~\ref{sec:evaluation}).
% \item Provided details on forecasting overhead (Section~\ref{sec:overhead}).
\item Updated Figure~\ref{fig:component-combined} and the related text to include additional data for different deadline constraints.
\item Made numerous editorial changes (figure sizes, captions, etc.) to improve readability. 
\end{itemize}

We also highlighted the changes with the yellow color in the paper.
Please note that, due to space constraints, some of the results (e.g.,  Figure~\ref{fig:dsvt_all}, Table~\ref{tab:allvelnumregionstest}, and Figures~\ref{fig:combined_deadlines}-\ref{fig:cp75valoall}) are included in the detailed responses rather than in the paper. 
Below, we provide detailed responses to the concerns raised by the reviewers. 

\subsection{Responses to Meta Review}

\subsubsection{On providing more details about region selection}
We provided additional details on our responses to Reviewer 1 (responses 3, 4, 5). 
We also revised Section~\ref{sec:region-sched} for clarification.

\subsubsection{On showing the miss rate comparison with Centerpoint100 and Centerpoint200}
We added Figure~\ref{fig:combined_deadlines}, which shows the miss rate comparison.

\subsubsection{On providing justification based on practical cases for the deadline constraints used in the paper}
Please refer to the first response to Reviewer 2.

\subsubsection{On comparing against other LiDAR object detection methods}
Please refer to the first response to Reviewer 4.


\subsection{Responses to Reviewer 1}

\subsubsection{On generalizability of VALO}

We chose the two specific architectures (CenterPoint and VoxelNext) for evaluation to showcase the generality of our approach as they represent very different network designs (one that uses a 2D backbone, while the other only utilizes sparse 3D convolutions). As we noted in the paper, however, our approach is generally applicable to any state-of-the-art 3D LiDAR-based object detection DNNs. 

VALO's generality stems from its ability to perform input data scheduling to make execution time and accuracy tradeoffs rather than requiring architectural modifications. As such, it can be generally applied to any 3D LiDAR-based detection models with different architectures.
To provide further evidence of VALO's generality, we apply it to another recent state-of-the-art transformer based 3D LiDAR objection model called Dynamic Sparse Voxel Transformer (DSVT) ~\footnote{H. Wang et al., "DSVT: Dynamic Sparse Voxel Transformer with Rotated Sets," IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), Vancouver, BC, Canada, 2023}. 

\begin{figure}[htp]  % You can use figure* for a wider figure if needed
    \centering

    \begin{subfigure}[b]{0.45\textwidth}  % Adjust the width as needed
        \includegraphics[width=\textwidth]{figures/response_letter/valo_dsvt_xavier/normalized_NDS_deadlines.pdf}
        \caption{Detection accuracies.}
        \label{fig:dsvt_acc}
    \end{subfigure}
    \hfill  % Add space between the subfigures
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/response_letter/valo_dsvt_xavier/deadlines_missed.pdf}
        \caption{Deadline miss rates.}
        \label{fig:dsvt_dl}
    \end{subfigure}
    \caption{Evaluation of VALO on DSVT}  % Add an overall caption
    \label{fig:dsvt_all}
\end{figure}
%\yun{I think it would be better to include a figure, say SECOND or DSVT result, whatever you tested}

Figure~\ref{fig:dsvt_all} shows the accuracy and deadline miss rates of the baseline DSVT and the VALO counterpart on a Jetson AGX Xavier platform.
%~\yun{why change the hardware platform without any explanation?}.
%~\fixme{AHMET: I am running the experiments on jetson agx now, we can decide which one to put once they finish} As can be seen in the figure, 
% the baseline DSVT fails to meet the deadline constraints and as a results deliver lower accuracy as the deadline get tigher. However, 
VALO can support a wide range of deadline constraints and as a result deliver higher accuracy over the baseline DSVT.
%VALO-applied DSVT clearly outperforms the baseline version, even without the need for training. 

%These include DNNs that apply sparse convolutions on voxels or pillars followed by dense convolutions (e.g. SECOND, CBGS, CenterPoint, PointPillars, PillarNet), DNNs that apply sparse convolutions only (e.g. VoxelNeXt), and DNNs that utilize transformers (e.g. TransFusion-L, DSVT). Figures

% \begin{figure}[htp]
% \centerline{\includegraphics[scale=0.6]{figures/response_letter/valo_dsvt_orin/normalized_NDS_deadlines.pdf}}
% \caption{Detection accuracies of VALO on DSVT.}
% \label{fig:dsvt_acc}
% \end{figure}

% \begin{figure}[htp]
% \centerline{\includegraphics[scale=0.6]{figures/response_letter/valo_dsvt_orin/deadlines_missed.pdf}}
% \caption{Deadline miss rates of VALO on DSVT.}
% \label{fig:dsvt_dl}
% \end{figure}


%VALO’s generalizability stems from its ability to perform input data scheduling from a bird-eye-view perspective (e.g. Figure~\ref{fig:partitioning}). It does not require any architectural modification to make execution time and accuracy tradeoffs.
%Only the detection head optimization (Section~\ref{sec:detheadopt}), which is not necessary to make tradeoffs, can require slight modification of DNN layers depending on its architecture, such as removing certain batch normalizations in CenterHead. If the detection head does not require any modification for optimization, a VALO-applied DNN does not require to be trained at all and can utilize the parameters (weights) of the baseline model. This is the case for VoxelNeXt.

\subsubsection{On the impact of forecasting and its overhead}

In our ablation study (Section~\ref{sec:ablationstudy}), we compared the baseline DNN with forecasting-enabled and forecasting-disabled versions of VALO-applied DNNs, illustrating the benefit of forecasting. The accuracy benefit is more significant when the deadline is tight since, in this case, fewer regions are processed in each frame, making the detection result more dependent on forecasted objects.

Regarding the timing overhead of forecasting compared to the baseline DNN, we observe negligible overhead (less than 1ms)
%we did not observe any overhead incurred by the forecasting operation itself when end-to-end latency is considered, 
as it is efficiently executed in parallel with the backbones. %However, we observed a 1 millisecond overhead on non-maximum suppression since forecasted objects are processed here together with the detected ones (Section~\ref{sec:detheadopt}).
%\yun{I think NMS of forecased objects is necessary computation, not overhead.}

\subsubsection{On whether regions are consistently considered vertical and the reasoning of it}

Yes, the regions are consistently considered vertical. We explored horizontal and tile-based partitioning but found vertical to be most effective. Horizontal regions are often non-empty and can't be skipped, while tile-based processing introduces significant overhead due to gather/scatter operations. Vertical partitioning, on the other hand, saves significant time in the 2D Backbone for many input frames by skipping empty vertical regions without sacrificing accuracy, as illustrated in Figure~\ref{fig:bb2dbp}.

\subsubsection{On how the number of regions is determined and its relationship with the operation environment}

We experimentally determined the number of regions. 
% The detection range and the number of regions are predetermined and fixed during runtime. We used the number 18 in our evaluation.
%To avoid tensor concatenation errors in the 2D backbone of the DNN, the number of regions must divide the width of all dense tensors evenly. 
While using more (thus, smaller) regions allows for finer-grained scheduling, it can increase runtime scheduling overhead and negatively impact the time prediction accuracy of the 3D backbone.
We find the number of regions, beyond a certain threshold, has a diminishing return as it makes little difference in overall accuracy. As for the impact of the operating environment such as the speed of the ego vehicle, we find that it does not have a noticeable impact in determining the the number of regions. 


\begin{table}[htp]
\centering
\caption{Detection accuracy of VALO-CP75 on Jetson AGX Xavier in different driving environments.}
%\yun{No need to have 2 digits subzero precision. You also forgot to mention how you performed the experiments.}}
%\yun{when the number of regions is too small or too large? as discussed, these tables are not sufficient. Also, what is the baseline accuracy you noramlized against and why the numbers are less than 90\%?} }
\label{tab:allvelnumregionstest}
\begin{subtable}{0.49\textwidth}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        Number of Regions & 2 & 5 & 9 & 18 & 30 & 90 \\ \hline
        %Average Accuracy (\%) & 66.5 & 84.5 & 88.1 & 87.4 & 87.9 & 88.2 \\ \hline
        Average NDS & 45.0 & 57.1 & 59.6 & 59.1 & 59.4 & 59.6 \\ \hline

    \end{tabular}
    \caption{Low-Speed Driving }
    \label{tab:lowvelnumregionstest}
\end{subtable}
\hfill
\begin{subtable}{0.49\textwidth}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        Number of Regions & 2 & 5 & 9 & 18 & 30 & 90 \\ \hline
        %Average Accuracy (\%) & 61.9 & 80.1 & 82.9 & 83.2 & 82.6 & 82.5 \\ \hline
        Average NDS & 40.2 & 52.0 & 53.9 & 54.1 & 53.6 & 53.6\\ \hline

    \end{tabular}
    \caption{High-Speed Driving}
    \label{tab:highvelnumregionstest}
\end{subtable}
\end{table}

Table~\ref{tab:allvelnumregionstest} shows the average accuracy results in nuScenes Detection Score (NDS) when using different numbers of regions on low- and high-speed scenes, respectively, of the nuScenes dataset. The results were obtained by taking the average of achieved NDS scores for the deadlines 90, 220, and 350 milliseconds.
Note, first, that, in both scenarios, when the number of regions is only 2, the accuracy is significantly lower. As we increase the number of regions, however, the accuracy improves. However, the improvements are plateaued after 9 regions. The results can be interpreted as follows. When the number of regions is too small, it limits the scheduler's ability to adapt to the different deadline constraints. After a certain number of regions, however, it has enough flexibility to meet various deadline constraints. We empirically chose 18 regions to give sufficient flexibility to the scheduler. 

%As shown, in both environments, the number of regions has minimal impact in overall accuracy results, suggesting it is not influenced by the environmental factor.

%Thus, the number of regions should be as much as possible while considering these constraints. 

% We tested VALO on the Centerpoint with a range of numbers of regions in two environments: low speed and high speed, and present the results in Table~\ref{tab:lowvelnumregionstest} and Table~\ref{tab:highvelnumregionstest}, respectively. The findings show that using 45 regions gave the best results in both environments, with less than \~1\% accuracy difference. This suggests that environmental conditions such as vehicle speed do not significantly impact the optimal number of regions. Since the accuracy difference between different region configurations was small, we used 18 regions in our experiments. This choice helped us to reduce the time needed for running the experiments by avoiding the increased initialization time required for DNN benchmarking operations (i.e. cuDNN benchmarking).



% \begin{table}[htp]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         Number of Regions & 10 & 15 & 18 & 30 & 45 \\ \hline
%         Normalized accuracy (\%) & 89.4 & 88.6 & 89.1 & 89.7 & 89.8 \\ \hline
%     \end{tabular}
%     \caption{Detection accuracy of VALO-CP75 in low-speed driving environment on Jetson AGX Xavier.}
%     \label{tab:lowvelnumregionstest}
% \end{table}

% \begin{table}[htp]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%         Number of Regions & 10 & 15 & 18 & 30 & 45 \\ \hline
%         Normalized accuracy (\%) & 85.3 & 85.4 & 85.1 & 85.2 & 85.3 \\ \hline
%     \end{tabular}
%     \caption{Detection accuracy of VALO-CP75 in high-speed driving environment on Jetson AGX Xavier.
%     \yun{when the number is regions is too small or too large? as discussed, these tables are not sufficient. Also, what is the baseline accuracy you noramlized against and why they are less than 90\%?}
% }
%     \label{tab:highvelnumregionstest}
% \end{table}


\subsubsection{On processing empty regions falling between non-empty regions}

The list of schedulable regions ($R_{S}$) can include empty regions, if they are surrounded by non-empty regions, to maintain spatial continuity. Excluding these empty regions could lead to non-adjacent regions being incorrectly treated as adjacent in the dense convolutions, negatively impacting the results. 

% Therefore, it's necessary to include empty regions that fall between non-empty ones.

\subsubsection{On the rationale of selecting the number of voxels in the most recent frames when doing the time prediction}

Our rationale for using the input voxel counts from the most recent previous frame is based on the observation that the similarity of voxel counts between two input frames increases as the time interval between them decreases. Since our predictions are made at the region level, for each candidate region \textit{r}, we specifically utilize the voxel counts observed the last time region \textit{r} was processed. We have revised Section~\ref{sec:time-pred} to clarify the mechanics and rationale of our method.

\subsubsection{On handling misprediction of execution time}

We employ the region dropping mechanism (Section~\ref{sec:region-drop}) to avoid missing deadlines in case of underpredicting the 3D backbone time ($E_S$).
Also, we already use the observed worst-case execution time for the last stage execution time ($E_R$) prediction, which helps handling underpredictions in the earlier stage.
%\fixme{AHMET: We don't have an underprediction problem for $E_D$}
%Also, using a constant worst-case execution time for $E_R$ creates a safe upper bound that covers many of the underpredictions. 
These mechanisms have been effective in preventing the need for overly pessimistic time predictions in all stages, which could waste resources and yield lower accuracy.

%Apart from these, we avoid making more pessimistic time predictions by adding a percentage as it results in wasting resources, yielding lower accuracy.

\subsubsection{On whether the forecast is done for a single or window of frames and about the details of forecasting queue maintenance}
It is the total number of detected objects in all input regions, not a window of frames, that determines the queue size. For all processed input regions of an input frame, VALO removes the old objects corresponding to these regions from the queue and appends the freshly detected objects in these regions to the queue. Thus, the queue maintains the latest detected objects of all regions.
%It is the total number of detected objects in the scene, not a window of frames, that determines the queue size. To calculate this, we track the latest number of objects detected in each input region. Summing the numbers for all regions gives the total number of objects, which defines the queue size. 
%Before each forecasting, we append all objects detected in the last frame, calculate the queue size, and adjust the queue to meet the limit.
%\yun{this is confusing. even after reading the algorithm you described in the google doc, it is still confusing.}
This ensures that the objects to be forecasted do not exceed the most recently known total number of objects detected in the scene.

A subset of the forecasted objects corresponds to the regions currently being processed, as we forecast objects from all regions. Possible duplicate results in these regions are eliminated through non-maximum suppression (NMS). NMS is configured to prioritize detected objects over forecasted ones if there is a bounding box overlap to prevent false positives.

\subsubsection{On missing deadline miss ratio figures}


\begin{figure}[htp]
    \centering 
    \begin{subfigure}{0.45\textwidth}  % Adjust width as needed
        \includegraphics[width=\textwidth]{figures/eval/jetson-xavier/set1/deadlines_missed.pdf}
        \caption{VALO vs. CenterPoint variants}
        \label{fig:dl2} 
    \end{subfigure}
    \hfill  % Add spacing between subfigures
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/eval/jetson-xavier/set3/deadlines_missed.pdf}
        \caption{VALO on VoxelNext}
        \label{fig:dl3}
    \end{subfigure}
    \hfill 
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/eval/jetson-xavier/set2/deadlines_missed.pdf}
        \caption{Variants of VALO}
        \label{fig:dl4}
    \end{subfigure}
    \caption{Deadline miss rate comparisons.} % Overall figure caption
    \label{fig:combined_deadlines} % Label for referencing the combined figure
\end{figure}

The requested deadline miss rate results are shown in Figure~\ref{fig:combined_deadlines}, which were omitted in the paper due to space limitations. Similar to Figure~\ref{fig:dl1}, VALO-applied DNNs avoid deadline misses thanks to its anytime computing capability. 
%In Figure~\ref{fig:dl3}, VALO experiences some deadline misses for tight deadlines because accurate time prediction (Section~\ref{sec:time-pred}) is more challenging for a fully sparse DNN like VoxelNext.
%reaching the limit of making tradeoffs and also 
%the more challenging time prediction (Section~\ref{sec:time-pred}) required for VoxelNext, as it is a fully sparse DNN.

\subsubsection{On the component-level execution time distributions for other deadlines}
We updated the results on Figure~\ref{fig:component-combined} to include 220 and 155 millisecond deadline constraints.

\subsubsection{On the missing definition \textit{c} in Eq.~\ref{eq:pose}}

It represents the confidence score of the object pose. We added the definition in the revision.

\subsection{Responses to Reviewer 2}

\subsubsection{On justifying evaluated deadline ranges}

According to literature~\cite{autoware}, the point clouds should be processed with a minimum frequency of 10 Hz (100ms/frame). Note that meeting such a deadline constraint is impossible for the baseline CenterPoint network on the evaluated hardware platform (Jetson AGX Xavier) as it takes more than 210ms even in the best case. VALO, on the other hand, make it possible to meet such a stringent deadline constraint with the highest possible accuracy under the constraint on the platform. On more powerful hardware (see Figure~\ref{fig:cp75valoall}, for example), VALO can support even more stringent deadlines. 

% Our choice of deadlines for evaluation is intended to stress the methods to make a fair comparison considering the computational limitations of the evaluation platform. For autonomous driving, the point clouds should be processed with a minimum frequency of 10 Hz~\cite{autoware} to the best of our knowledge. VALO makes this possible on Jetson AGX Xavier and also enables higher frequencies on stronger platforms such as Jetson AGX Orin.

\subsubsection{On having a section for the training hyperparameters and releasing the code}

When training the VALO applied CenterPoint, we used the same hyperparameters of the baseline available in the OpenPCDet~\cite{openpcdet2020}, which our work is extended on.
For VALO applied VoxelNext, we did not train the model and instead used the pretrained baseline model in the OpenPCDet repository.
Our code will be available on a public GitHub repository with step-by-step instructions to reproduce all presented results.

\subsubsection{On the performance requirements of 3D backbone when SECOND~\cite{second} and TorchSparse~\cite{torchsparse} are used}

SECOND~\cite{second} is one of the baseline 3D object detection models, which is already supported in OpenPCDet. 
TorchSparse~\cite{torchsparse}, on the other hand, is an alternative sparse convolution library. However, the latest SpConv v2.3.6 library used in OpenPCDet is known to be faster than TorchSparse.
Note that VALO can be applied to any LiDAR-based object detection model supported by the OpenPCDet framework.
%The 3D backbone of~\cite{second} is the same one used in CenterPoint. 
%Since OpenPCDet has no support for~\cite{torchsparse}, we tested with the supported \textit{spconv} library and used its latest version (v2.3.6). Spconv provides highly optimized sparse convolutions on GPU similar to~\cite{torchsparse}, thus we expect the results to be similar.

\subsubsection{On VALO's performance on high-end systems}

We also tested VALO on a Jetson Xavier Orin and a desktop computer equipped with an NVIDIA RTX 3080 GPU. On both platforms, VALO proved effective, achieving the highest accuracy under a wide range of deadline constraints. Figure~\ref{fig:cp75valoall} compares VALO's performance to CenterPoint baselines on the two high-end platforms.


% \begin{figure}[htp]
% \centerline{\includegraphics[scale=0.6]{figures/response_letter/martian_eval/set0/martian_normalized_NDS_deadlines_set0.pdf}}
% \caption{Detection accuracies when comparing anytime computing methods with the baseline CenterPoint75 on the high-end system. \yun{I don't think we need to include this figure. Figure~\ref{fig:martian2} should be sufficient for the RTX 3080 results.}}
% \label{fig:martian1}
% \end{figure}

% \begin{figure}[htp]
% \centerline{\includegraphics[width=0.45\textwidth]{figures/response_letter/martian_eval/set1/normalized_NDS_deadlines.pdf}}
% \caption{Detection accuracies of VALO and the CenterPoint baselines on the high-end system (NVIDIA RTX 3080 + Intel Core i7-11700KF).}
% \label{fig:martian2}
% \end{figure}

\begin{figure}[htp]  % You can use figure* for a wider figure if needed
    \centering

    \begin{subfigure}[b]{0.45\textwidth}  % Adjust the width as needed
        \includegraphics[width=\textwidth]{figures/response_letter/martian_eval/set1/normalized_NDS_deadlines.pdf}
        \caption{On NVIDIA RTX 3080 + Intel Core i7-11700KF.}
        \label{fig:cp75valomartian}
    \end{subfigure}
    \hfill  % Add space between the subfigures
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/response_letter/valo_cp75_orin/normalized_NDS_deadlines.pdf}
        \caption{On Jetson AGX Orin.}
        \label{fig:cp75valoorin}
    \end{subfigure}
    \caption{Detection accuracies of VALO and the CenterPoint baselines on the high-end systems.}  % Add an overall caption
    \label{fig:cp75valoall}
\end{figure}

\subsection{Responses to Reviewer 3}

\subsubsection{On the effect of different datasets}

The nuScenes dataset~\cite{nuscenes} we used in this paper is a large-scale dataset, covering diverse driving scenarios. It is a representative and widely used dataset for autonomous driving research, which is why we chose it for our study. However, we believe our approach is generally applicable irrespective of the dataset.

\subsubsection{On the definition of normalized accuracy}
To better present the accuracy of each method relative to others, we normalized the obtained NDS of all methods by dividing them with the maximum NDS observed among the methods being compared. We added this definition in Section~\ref{sec:evaluation}.

\subsubsection{On providing an example for anytime computing in the background}
We added an example of an anytime path planning algorithm~\cite{boddy1989solving} to the background section.
%\yun{I am not sure of this example. I feel it is unnecessarily long.}

\subsection{Responses to Reviewer 4}
\subsubsection{On comparing against other LiDAR object detection methods that trade off accuracy with time}

In the related work section of~\cite{alidar}, the anytime methods that were discussed apply to 2D image processing DNNs and do not apply to LiDAR object detection DNNs. To the best of our knowledge, AnytimeLidar~\cite{alidar} is the only other LiDAR-based anytime object detection method. 
%~we can directly compare against. 

%Thus, we compared against the only available anytime method for LiDAR

\subsubsection{On why our greedy scheduling policy works well}
%I copied this paragraph from the paper. Do you think we need to paraphrase it?
Using this policy brings three advantages. Firstly, selecting adjacent regions maintains spatial continuity and processes the input with minimal fragmentation, thereby avoiding accuracy degradation that can happen through slicing and batching nonadjacent regions. Secondly, it ensures a consistent level of ``freshness'' of object detection results over all regions, which is needed for effective forecasting operations. Thirdly, it incurs minimal scheduling overhead.

% VALO does not enforce this scheme and is upgradeable to more sophisticated solutions. We leave it as a future work to explore such solutions.

% \subsection{Revisions}


==> sections/algos/h2.tex <==
\setlength{\textfloatsep}{2pt}
\begin{algorithm}[t]
\DontPrintSemicolon
\textbf{Input}:\\
List of Input Voxels ($L$),\\
Number of Input Regions ($N_R$),\\
History Buffer ($H$),\\
\textbf{Output}: Selected Regions to be Processed\\
%\nonl\;
\SetKwProg{funct}{function}{}{}
\SetKwFunction{func}{update_buffer}

\funct{\func{$L$, $N_R$, $H$}}
{
    $i \gets 0$
    \For{each item $V$ in $L$}
    {
        $R_{S}, C_{S} \gets count\_features(V, N_R)$\\
        $H[i, R_{S}] = C_{S}$\\
        $i \gets i + 1$
    }
}
\Return{$R_{sel}$}
\caption{Voxel history buffer update algorithm}
\label{alg:algo1}
\end{algorithm}

==> sections/figs/edge_prob.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.70\linewidth]{figures/edge_probability_light.pdf}
	\caption{Impact of edge probability on virtual gang formation for lightly parallel tasksets}
	\label{fig:ev-edgeprob}
\end{figure}

==> sections/figs/sched_plot_p0.tex <==
\begin{figure*}[t]
    \centering % <-- added
\medskip
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/light_e0_rr.pdf}
  \caption{Lightly Parallel}
  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/mixed_e0_rr.pdf}
  \caption{Mixed}
  \label{fig:5}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/heavy_e0_rr.pdf}
  \caption{Heavily Parallel}
  \label{fig:6}
\end{subfigure}
\caption{Schedulability plots for tasksets containing independent tasks ($P(e) = 0$) on 8 cores.}
%Dashed lines are used when interference is not considered. For RT-Gang, because only one task can be scheduled at a time, interference cannot occur by design (thus no dashed lines)}
% \vspace*{-5mm}
\label{fig:sim-p0}
\end{figure*}

==> sections/figs/sched_plot_p25.tex <==
\begin{figure*}[t]
    \centering % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/light_e25_rr.pdf}
  \caption{Lightly Parallel}
  \label{fig:1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/mixed_e25_rr.pdf}
  \caption{Mixed}
  \label{fig:2}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.28\textwidth}
  \includegraphics[height=3.5cm,width=\linewidth]{figures/heavy_e25_rr.pdf}
  \caption{Heavily Parallel}
  \label{fig:3}
\end{subfigure}
\caption{Schedulability plots for tasksets with precedence constraints ($P(e) = 0.25$) on 8 cores}
% \vspace*{-5mm}
\label{fig:sim-p25}
\end{figure*}

==> sections/figs/smt_timing.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[height=4.5cm, width=0.75\linewidth]{figures/smt_timing_box.pdf}
	\caption{Comparison of SMT and heuristic virtual gang formation runtime. In each box, the orange line represents the median value. The box represents the interquartile range (Q2-Q3). The lower and upper whiskers mark the 5 percentile and the 95 percentile values respectively.}
	\label{fig:smt-time}
\end{figure}
